Empir3D : A Framework for Multi-Dimensional Point Cloud Assessment

Advancements in sensors, algorithms, and compute hardware have made 3D perception feasible in real time. Current methods to compare and evaluate the quality of a 3D model, such as Chamfer, Hausdorff, and Earth-Mover's distance, are uni-dimensional and have limitations, including an inability to capture coverage, local variations in density and error, and sensitivity to outliers. In this paper, we propose an evaluation framework for point clouds (Empir3D) that consists of four metrics: resolution to quantify the ability to distinguish between individual parts in the point cloud, accuracy to measure registration error, coverage to evaluate the portion of missing data, and artifact score to characterize the presence of artifacts. Through detailed analysis, we demonstrate the complementary nature of each of these dimensions and the improvements they provide compared to the aforementioned uni-dimensional measures. Furthermore, we illustrate the utility of Empir3D by comparing our metrics with uni-dimensional metrics for two 3D perception applications (SLAM and point cloud completion). We believe that Empir3D advances our ability to reason about point clouds and helps better debug 3D perception applications by providing a richer evaluation of their performance. Our implementation of Empir3D, custom real-world datasets, evaluations on learning methods, and detailed documentation on how to integrate the pipeline will be made available upon publication.

==> archive.tex <==
% \section{PROCEDURE FOR PAPER SUBMISSION}

% \subsection{Selecting a Template (Heading 2)}

% First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
% It may be used for A4 paper size if the paper size setting is suitably modified.

% \subsection{Maintaining the Integrity of the Specifications}

% The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

% \section{MATH}

% Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

% Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

% \subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

% \subsection{Units}

% \begin{itemize}

% \item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as Ò3.5-inch disk driveÓ.
% \item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
% \item Do not mix complete spellings and abbreviations of units: ÒWb/m2Ó or Òwebers per square meterÓ, not Òwebers/m2Ó.  Spell out units when they appear in text: Ò. . . a few henriesÓ, not Ò. . . a few HÓ.
% \item Use a zero before decimal points: Ò0.25Ó, not Ò.25Ó. Use Òcm3Ó, not ÒccÓ. (bullet list)

% \end{itemize}


% \subsection{Equations}

% The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

% $$
% \alpha + \beta = \chi \eqno{(1)}
% $$

% Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use Ò(1)Ó, not ÒEq. (1)Ó or Òequation (1)Ó, except at the beginning of a sentence: ÒEquation (1) is . . .Ó

% \subsection{Some Common Mistakes}
% \begin{itemize}


% \item The word ÒdataÓ is plural, not singular.
% \item The subscript for the permeability of vacuum ?0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ÒoÓ.
% \item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
% \item A graph within a graph is an ÒinsetÓ, not an ÒinsertÓ. The word alternatively is preferred to the word ÒalternatelyÓ (unless you really mean something that alternates).
% \item Do not use the word ÒessentiallyÓ to mean ÒapproximatelyÓ or ÒeffectivelyÓ.
% \item In your paper title, if the words Òthat usesÓ can accurately replace the word ÒusingÓ, capitalize the ÒuÓ; if not, keep using lower-cased.
% \item Be aware of the different meanings of the homophones ÒaffectÓ and ÒeffectÓ, ÒcomplementÓ and ÒcomplimentÓ, ÒdiscreetÓ and ÒdiscreteÓ, ÒprincipalÓ and ÒprincipleÓ.
% \item Do not confuse ÒimplyÓ and ÒinferÓ.
% \item The prefix ÒnonÓ is not a word; it should be joined to the word it modifies, usually without a hyphen.
% \item There is no period after the ÒetÓ in the Latin abbreviation Òet al.Ó.
% \item The abbreviation Òi.e.Ó means Òthat isÓ, and the abbreviation Òe.g.Ó means Òfor exampleÓ.

% \end{itemize}


% \section{USING THE TEMPLATE}

% Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

% It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

% \subsection{Headings, etc}

% Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named ÒHeading 1Ó, ÒHeading 2Ó, ÒHeading 3Ó, and ÒHeading 4Ó are prescribed.

% \subsection{Figures and Tables}

% Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text. Use the abbreviation ÒFig. 1Ó, even at the beginning of a sentence.

% \begin{table}[h]
% \caption{An Example of a Table}
% \label{table_example}
% \begin{center}
% \begin{tabular}{|c||c|}
% \hline
% One & Two\\
% \hline
% Three & Four\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}


%    \begin{figure}[thpb]
%       \centering
%       \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
% }}
%       % \includegraphics[scale=1.0]{image.png}
%       \caption{Inductance of oscillation winding on amorphous
%        magnetic core versus DC bias magnetic field}
%       \label{figurelabel}
%    \end{figure}
   

% Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity ÒMagnetizationÓ, or ÒMagnetization, MÓ, not just ÒMÓ. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write ÒMagnetization (A/m)Ó or ÒMagnetization {A[m(1)]}Ó, not just ÒA/mÓ. Do not label axes with a ratio of quantities and units. For example, write ÒTemperature (K)Ó, not ÒTemperature/K.Ó

% \section{CONCLUSIONS}

% A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

% \addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
%                                   % on the last page of the document manually. It shortens
%                                   % the textheight of the last page by a suitable amount.
%                                   % This command does not take effect until the next page
%                                   % so it should come on the page before the last. Make
%                                   % sure that you do not shorten the textheight too much.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{APPENDIX}

% Appendixes should appear before the acknowledgment.

% \section*{ACKNOWLEDGMENT}

% The preferred spelling of the word ÒacknowledgmentÓ in America is without an ÒeÓ after the ÒgÓ. Avoid the stilted expression, ÒOne of us (R. B. G.) thanks . . .Ó  Instead, try ÒR. B. G. thanksÓ. Put sponsor acknowledgments in the unnumbered footnote on the first page.



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.




% \begin{thebibliography}{99}

% \bibitem{c1} G. O. Young, ÒSynthetic structure of industrial plastics (Book style with paper title and editor),Ó 	in Plastics, 2nd ed. vol. 3, J. Peters, Ed.  New York: McGraw-Hill, 1964, pp. 15Ð64.
% \bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123Ð135.
% \bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
% \bibitem{c4} B. Smith, ÒAn approach to graphs of linear forms (Unpublished work style),Ó unpublished.
% \bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
% \bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
% \bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
% \bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ÒElectron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),Ó IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740Ð741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
% \bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
% \bibitem{c10} J. U. Duncombe, ÒInfrared navigationÑPart I: An assessment of feasibility (Periodical style),Ó IEEE Trans. Electron Devices, vol. ED-11, pp. 34Ð39, Jan. 1959.
% \bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ÒA clustering technique for digital communications channel equalization using radial basis function networks,Ó IEEE Trans. Neural Networks, vol. 4, pp. 570Ð578, July 1993.
% \bibitem{c12} R. W. Lucky, ÒAutomatic equalization for digital communication,Ó Bell Syst. Tech. J., vol. 44, no. 4, pp. 547Ð588, Apr. 1965.
% \bibitem{c13} S. P. Bingulac, ÒOn the compatibility of adaptive controllers (Published Conference Proceedings style),Ó in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8Ð16.
% \bibitem{c14} G. R. Faulhaber, ÒDesign of service systems with priority reservation,Ó in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3Ð8.
% \bibitem{c15} W. D. Doyle, ÒMagnetization reversal in films with biaxial anisotropy,Ó in 1987 Proc. INTERMAG Conf., pp. 2.2-1Ð2.2-6.
% \bibitem{c16} G. W. Juette and L. E. Zeffanella, ÒRadio noise currents n short sections on bundle conductors (Presented Conference Paper style),Ó presented at the IEEE Summer power Meeting, Dallas, TX, June 22Ð27, 1990, Paper 90 SM 690-0 PWRS.
% \bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
% \bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
% \bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
% \bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 



% \end{thebibliography}








% \section{Experimental Evaluation}
% \label{eval_section}

% PQM is implemented using Open3D \cite{Zhou2018} and PDAL  \cite{pdalcontributorsPDALPointData2020} libraries and runs entirely on a desktop workstation with 6c/12t CPU and 32 GB of Memory. We also provide a CUDA accelerated implementation with PyTorch \cite{NEURIPS2019_9015} which can be advantageous for large point clouds.

% % \subsection{Datasets}


% % \input{sections/tables/ablation_table}

% Experimental evaluation is performed on three simulation datasets, the HILTI dataset \cite{zhangHiltiOxfordDatasetMillimetreAccurate2022} and the Stanford bunny \cite{bunny}

% Experiments were conducted on 3 simulation datasets collected using a gazebo based simulation environment \textbf{more on this}, on one sequence of the HILTI  and the Stanford bunny point cloud dataset.




% \subsection{Ablation Study}
% \label{ablation_eval}


% %    \begin{figure}[htbp]
% %       \centering
% %       \begin{tabular}{c|c|c|c}
% % %       \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
% % % }}
% %       \includegraphics[width=200px, height=150px]{images/bunny/add_artifacts.png} &
% %       \includegraphics[width=200px, height=150px]{images/bunny/remove_completeness.png} &
% %       \includegraphics[width=200px, height=150px]{images/bunny/voxel_resolution.png} &
% %       \includegraphics[width=200px, height=150px]{images/bunny/gaussian_accuracy.png}
% %       \caption{Bunny plots}
% %       \label{bunny_plot}
% %       \end{tabular}
% %    \end{figure}



% \begin{figure*}[htbp]
%    \centering
%    \begin{tabular}{cccc}

%   %  \includegraphics[width=0.23\textwidth,height=5cm]{images/bunny_plots/add_leg_correct.png} &
%   % \includegraphics[width=0.23\textwidth,height=5cm]{images/bunny_plots/remove_leg_correct.png} &
%   % \includegraphics[width=0.23\textwidth,height=5cm]{images/bunny_plots/gaussian_leg_correct.png} &
%   \includegraphics[width=\textwidth]{images/bunny/bunny_damage_plots_combined.pdf} \\
%       % (a) Add (Artifacts) & (b) Remove (Completeness) & (c) Gaussian (Accuracy) & (d) Downsample (Resolution) 
%    \end{tabular}
%    \caption{Bunny plots; left to right: Add, Remove, Gaussian, Down-sample }
%    \label{bunny_plot}
% \end{figure*}



% % \begin{figure*}[htbp]
% %    \centering
% %    \begin{tabular}{cccc}

% %   %  \includegraphics[width=0.23\textwidth,height=5cm]{images/bunny_plots/add_leg_correct.png} &
% %   % \includegraphics[width=0.23\textwidth,height=5cm]{images/bunny_plots/remove_leg_correct.png} &
% %   % \includegraphics[width=0.23\textwidth,height=5cm]{images/bunny_plots/gaussian_leg_correct.png} &
% %   \includegraphics[width=\textwidth]{images/bunny/ref_metric_damage.pdf} \\
% %       % (a) Add (Artifacts) & (b) Remove (Completeness) & (c) Gaussian (Accuracy) & (d) Downsample (Resolution) 
% %    \end{tabular}
% %    \caption{Reference metric on Bunny}
% %    \label{ref_metric_plot}
% % \end{figure*}

% \input{sections/tables/ablation_slam_table}


% %    \begin{figure*}[!h]
% %       \centering
% % %       \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
% % % }}
% %       \includegraphics[width=\textwidth]{images/warehouse_section_qualitative5.jpeg}
% %       \caption{Qualitative Analysis}
% %       \label{figurelabel}
% %    \end{figure*}

% \begin{figure*}[htbp]
%   \begin{center}
%   \includegraphics[width=\textwidth]{images/map_grid_label.pdf}
%   \caption{Evaluation on SLAM systems. Left to right (Worlds) : Mai City, Warehouse, Village, HILTI \\ 
%   Top to bottom : Puma, FAST-LIO2, LeGO-LOAM, Ground Truth   \yash{Increase font and bold}}

%   \label{slam-maps}
%     \end{center}
% \end{figure*}



% % \input{sections/tables/slam_table}
% \input{sections/tables/hilti_table}
% % \input{sections/tables/slam_hilti_combined}
% \fixed{Need to make all references consistent Fig. Fig[] etc...}
% To evaluate the performance of PQM in isolation we "degraded" the Stanford bunny \cite{bunny} point cloud as described in SEC. \ref{ablation_method}. \tent{
% by : adding points, removing points, applying Gaussian noise to existing points and down-sampling. Each type of degradation, targets \tent{degradation to one} a specific sub-metric SEC.\ref{pqm_method}, i.e Artifacts, Completeness, Accuracy and Resolution. 
% }
% \fixed{Should we use $pcdA$ nomenclature instead of GT and cand / degraded in this case - $pcd_{B}$}. Experiments were performed for a range of degradation in the percent of points to be affected (0\% to 90\% with an increment of 5\%,total 19 values), except for down-sampling, where we use degradation parameter as sample rate (1 to 19 with an increment of 1, total 19, for consistency with percent results). Further, \tent{extending the dimension of the experiment,} we also performed the \tent{whole} experiment for different cell sizes i.e 0.05, 0.04, 0.03, 0.02 (meter). The results for the degradation experiments with cell size 0.05 (dividing the model into 4x4x3 cells) are shown in Fig. \ref{bunny_plot}. The parameter $\epsilon$ is computed and maintained as half the average distance between points in $pcd_{A}$, which is a reasonable estimate for a valid points threshold. $\epsilon$ is a tuneable parameter and can be decided based on application. All the plots are evaluated with \tent{cell size of 0.05m and} weights $\omega_c, \omega_t,\omega_a$ and $\omega_r = 0.25$, and $\epsilon = 0.0002$.
 
% \tent{Following are the explanation of effect of each degradation type:}
% \yash{Check for overlap with degradation explanation in \ref{method}}
% \subsubsection{Artifact Score} 
% \label{add_eval}
% As shown in Tab. \ref{table_ablation}, \tent{first 3 entries,} adding artifacts  \tent{ with different percent (25,50,75)} proportionally decreases the \tent{  artifact sub-metric score}  $\qt{}$ , while $\qa{}$ and $\qc{}$ are unchanged. Consequently $\qr{}$ is affected, due to the fact that adding a spherical artifact in each cell increases the volume of the point cloud, reducing the resolution. The Fig. \ref{bunny_plot} shows the artifact score decreasing proportional to the percent of points added, affecting overall quality $\qq{}$.  

% \fixed{Changing subsections to target submetrics}
% \subsubsection{Completeness} 
% \label{remove_eval}
% \tent{Points are removed to target completeness, in each cell a continuous patch of specified percent of points are removed using K-Nearest Neighbor method.} 
% As seen in Tab.\ref{table_ablation}, \tent{for damage type "Remove" with percent(25,50,75),} completeness score $\qc{}$ is decreases proportional to the percent of degradation applied. The Fig. \ref{bunny_plot} shows the same \tent{completeness value going down proportional to the percent of points removed,} resulting in overall $\qq{}$ decrease. Additionally, this also affects the resolution due to number of points reduced but volume is unchanged, decreasing the $\qr{}$ score while $\qa{}$  and $\qt{}$ are unchanged.


% \subsubsection{Accuracy} 
% \label{gauss_eval}
% \tent{Here, we target the accuracy sub-metric degradation with control parameter as percent of points in a cell is applied by applying Gaussian noise with $\mu$ as zero and}
% We used $\sigma$ constrained to euclidean distance of $\epsilon$(i.e. 0.0002m). The reason for calculating $\sigma$ in this manner is, if noise is applied higher than $\epsilon$, number of valid points decrease affecting completeness and artifact score. Tab. \ref{table_ablation}\tent{damage type "Gaussian" with percent(25,50,75),} shows  $\qa{}$ is the only sub-metric affected, resulting in $\qq{}$ score decrease. Other sub-metrics negligibly changed due \tent{to the reason that, } to the fact that only a few boundary points \yash{frame better - overflow? }may have gone out of a cell. This also proves the efficacy of PQM for small changes. Fig. \ref{bunny_plot} shows a clear  decrease in accuracy, as \tent{higher percent of points as applied a} Gaussian noise is increased.\tent{ Also we can see other sub-metric fluctuating due to the effect of Gaussian noise on boundary points explained above.}


% \subsubsection{Resolution} 
% \label{downsample_eval}
% \tent{Down-sampling targets resolution by uniformly sampling the point cloud at a specified sampling rate.} Tab.\ref{table_ablation} \tent{damage type "Downsample" with sample rates(5, 10, 15),} shows resolution is decreasing with increase in sampling rate. This is unlike \ref{remove_eval} \tent{experiment is different than "Remove" degradation,} as removing continuous patch of points affects completeness more than resolution, while down-sampling degrades $\qr{}$ and $\qc{}$ almost equally, if not exactly as seen in Fig. \ref{bunny_plot}. \tent{ And there is no way, we can affect $\qr{}$ specifically without affecting $\qc{}$. Fig.\ref{bunny_plot} Downsample also shows the down-sampling correlation with the $\qr{}$ score and consequently $\qc{}$ score. }

% \subsubsection{\cd{} and \hd{} Distance}
% \label{cd_hd_eval}
% Fig. \ref{bunny_plot}, shows the \cd{} and \hd{} for the four degradations performed same as used for evaluating PQM in Sec.\ref{ablation_eval}. \cd{} (green) shows gradual increase in value, which signifies increasing degrade in quality, but it fails to give insights about type of quality that is affected. Additionally, its value is unbounded, and hence cannot justify normalized quality value for a reasonable comparison. In the case of \hd{} (blue), values do not show any correlation with the applied degradation.

% The results of these experiments show that PQM is effective in detecting and quantifying changes in map quality due to different types and levels of degradation. The scores generated by PQM highly correlate with the expected change in resulting value for each targeted sub-metric.

% Overall, the experiment demonstrated the effectiveness of PQM metric in evaluating the quality of point clouds and detecting changes in map quality due to different types and levels of degradation \tent{. The results of the experiment shows that our metric is suitable to capture different aspects of map quality, }and hence can act as a tool to detect point cloud suitability for specific applications.


% \yash{we're saying we calculate $\epsilon$ based on average distance but we dont do this for SLAM tests - explain! - one way is to be consistent across larger maps we chose 0.1 and etc ...}


% \subsection{Evaluation on SLAM systems}
% \label{slam_eval}

% % Exhaustive evaluation on maps generated using the SLAM systems mentioned above in 3 simulation worlds and exp04 sequence of the HILTI dataset demonstrates the performance of PQM on large realistic point cloud maps. Fig. \ref{slam-maps} shows the qualitative differences between maps generated by the SLAM systems compared to ground truth. 
% % Tab. \ref{slam_table} shows the sub-metrics for each map, each sub-metric evaluates a certain aspect of quality as defined in Sec.\ref{method}. PQM is computed as the weighted sum of the sub-metrics where the weights (Eq. \ref{pqm}) are set by the user based on target application. For all evaluation weights are set to $0.25$ making the contribution of each sub-metric equal for over-all quality. We also set $\epsilon = 0.1$ and cell size $r = 10$ for all tests in Tab. \ref{slam_table}, more suitable values were not explored for all maps due to the long computing times. A study of the effect of $\epsilon$ and $r$ is shown in Tab. \ref{hilti_table}

% % Although it is visually apparent that FAST-LIO2 generates the highest quality maps compared to the other methods in terms of resolution, completeness and accuracy, this is not reflected in the highlighted chamfer and hausdorff distance values in Tab. \ref{slam_table}. We can see that chamfer and hausdorff distances only correctly identify the best map 1/4 and 0/4 times respectively. 
% % PQM on the other hand consistently identifies point clouds generated by FAST-LIO2 as the ones with highest overall quality. The sub-metrics are also indicative of PQM's performance with only $\qa{}$ being incorrect in 2 instances, HILTI and Warehouse. This is likely due to the threshold of $\epsilon = 0.1$ used. A lower $\epsilon$ value will correctly identify $\qa{}$, this is seen in Tab. \ref{hilti_table}. Highlighted values show that as $\epsilon$ is reduced (0.01) quality is calculated correctly 2/3 times which is much better given higher values miss it almost every time. 

% \yash{Mention varying $\epsilon$ and size - very little efferct on PQM}
% % Gen Test
% The performance of PQM on large, realistic point cloud maps generated using the SLAM systems mentioned above was evaluated exhaustively in three simulation worlds and the exp04 sequence of the HILTI dataset. The results of this evaluation are presented in Fig. \ref{slam-maps}, which shows the qualitative differences between the maps generated by the SLAM systems and the ground truth. Tab. \ref{slam_table} shows the sub-metrics for each map. Each sub-metric evaluates a certain aspect of quality as defined in Sec. \ref{method}. PQM is computed as the weighted sum of these sub-metrics, where the weights (Eq. \ref{pqm}) are set by the user based on the target application. \verify{For all evaluations, the weights were set to 0.25, making the contribution of each sub-metric equal for overall quality.} We also set $\epsilon = 0.1$ and cell size $r = 10$ for all tests in Tab. \ref{slam_table}. More suitable values were not explored for all maps due to long computing times. \verify{A study of the effect of $\epsilon$ and $r$ is shown in Tab. \ref{hilti_table}.}

% Visually, it is apparent that the FAST-LIO2 SLAM system generates the highest-quality maps compared to the other methods in terms of resolution, completeness, and accuracy. However, the highlighted \cd{} and \hd{} distance values in Tab. \ref{slam_table} do not reflect this observation. We can see that \cd{} and \hd{} distances only correctly identify the best map 1/4 and 0/4 times, respectively.

% On the other hand, PQM consistently identifies point clouds generated by FAST-LIO2 as the ones with the highest overall quality. The sub-metrics are also indicative of PQM's performance, with only $\qa{}$ being incorrect in 2 instances (HILTI and Warehouse). \verify{This is likely due to the threshold of $\epsilon = 0.1$ used. However, a lower $\epsilon$ value will correctly identify $\qa{}$, as seen in Tab. \ref{hilti_table}. Highlighted values show that as $\epsilon$ is reduced (to 0.01), quality is calculated correctly 2/3 times, which is much better given that higher values miss it almost every time.}

% \yash{Do we add table 3? if we show that lower $\epsilon$ leads to better accuracy estimate then readers might ask why didn't we use a lower one in the first place - one answer is it takes time to find a good value ... etc}



% % \subsubsection{Runtime and Computational Performance}
% % \textbf{@PRANAY can you do this?  -  Also not sure if we should include}



==> latexmkrc <==
$sub_doc_output = '.';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-f",
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> use-cases.tex <==
\section{Applications}

In this section we show how PQM can be used for point cloud analysis beyond trivial quality evaluation. First, we evaluate a point cloud object-detection method \yash{cite} for its performance on point clouds with varying resolution and coverage. This can help identify sensors and representations that maximize object detection confidence for a particular scene / object class. 

Second, we demonstrate PQM's use in quantitatively measuring the increase in coverage for an infrastructure assisted perception system for autonomous driving applications. This system involves a LiDAR sensor installed at a busy intersection which shares scans with an incoming autonomous vehicle to increase the vehicle's effective field-of-view (E-FOV). While we can subjectively confirm the increase in E-FOV, precise measurement of the increase in E-FOV can help identify the optimal pose for the infrastructure and vehicle sensors.
\begin{figure}
  \centering
  % \includegraphics[trim=1cm 1cm 1cm 1cm,clip=true,width=.9\columnwidth]{images/RLV_RSS_Coverage.pdf}
  \includegraphics[width=\columnwidth]{images/RLV_RSS_Coverage.pdf}
  \caption{Figure shows increase in coverage }
  \label{RLV_Coverage}
  % \vspace{-0.7cm}
\end{figure}

\yash{ref fig.} shows the increase in coverage seen by combining the infrastructure point cloud with the vehicle point cloud. It is evident that fusing the two point clouds increase the E-FOV of the vehicle by a constant value of 6\% (\(\qc{} = 0.06\)) which can assist the autonomous vehicle by allowing it to see around corners and make life-saving decisions early-on.



It is important to note that this evaluation is targeted to demonstrate PQM's use beyond 
